Algorithm-agnostic significance testing in supervised learning with multimodal data

Valid statistical inference is crucial for decision-making but difficult to obtain in supervised learning with multimodal data, e.g., combinations of clinical features, genomic data, and medical images. Multimodal data often warrants the use of black-box algorithms, for instance, random forests or neural networks, which impede the use of traditional variable significance tests. We address this problem by proposing the use of COvariance Measure Tests (COMETs), which are calibrated and powerful tests that can be combined with any sufficiently predictive supervised learning algorithm. We apply COMETs to several high-dimensional, multimodal data sets to illustrate (i) variable significance testing for finding relevant mutations modulating drug-activity, (ii) modality selection for predicting survival in liver cancer patients with multiomics data, and (iii) modality selection with clinical features and medical imaging data. In all applications, COMETs yield results consistent with domain knowledge without requiring data-driven pre-processing which may invalidate type I error control. These novel applications with high-dimensional multimodal data corroborate prior results on the power and robustness of COMETs for significance testing. COMETs are implemented in the comets R package available on CRAN and pycomets Python library available on GitHub. Source code for reproducing all results is available at https://github.com/LucasKook/comets. All data sets used in this work are openly available.

==> Fig/varsig.tex <==
\fbox{%
\begin{tikzpicture}[auto, Arr/.style={-{Latex[length=1.5mm]}}]
\node (a2) {\textbf{\textsf{Variable significance}}};
\node[below=0cm of a2] (h03) {$H_0: Y \indep X_j \mid X_{-j}, Z$};
\node[below=0cm of h03] {\includegraphics[width=3.5cm]{Fig/manhatten.pdf}};
\end{tikzpicture}%
}
